Robust Graph Clustering via Meta Weighting for Noisy Graphs

How can we find meaningful clusters in a graph robustly against noise edges? Graph clustering (i.e., dividing nodes into groups of similar ones) is a fundamental problem in graph analysis with applications in various fields. Recent studies have demonstrated that graph neural network (GNN) based approaches yield promising results for graph clustering. However, we observe that their performance degenerates significantly on graphs with noise edges, which are prevalent in practice. In this work, we propose MetaGC for robust GNN-based graph clustering. MetaGC employs a decomposable clustering loss function, which can be rephrased as a sum of losses over node pairs. We add a learnable weight to each node pair, and MetaGC adaptively adjusts the weights of node pairs using meta-weighting so that the weights of meaningful node pairs increase and the weights of less-meaningful ones (e.g., noise edges) decrease. We show empirically that MetaGC learns weights as intended and consequently outperforms the state-of-the-art GNN-based competitors, even when they are equipped with separate denoising schemes, on five real-world graphs under varying levels of noise. Our code and datasets are available at https://github.com/HyeonsooJo/MetaGC.

==> 031analysis.tex <==
Recall that the objective function of \Ours (i.e., Eq.~\eqref{eq:overall_loss}) is based on modularity.
In this section, we show that when soft cluster assignment matrices are used,  modularity-based objectives are suitable for direct continuous relaxation,
% (i.e., a continuous relaxation),
while normalized-cut-based objectives are unsuitable.
Given a graph $G$ and a soft cluster assignment matrix $P \in [0, 1]^{N \times K}$,
recall that we can interpret each entry $P_{ix}$ of $P$ as the probability that we assign node $v_i$ to cluster $x$.
From another perspective, we may see $P$ as a random variable taking values in $\mathcal{P}^*$,
then the probability that $P$ corresponds to a deterministic cluster assignment matrix $P^* \in \{0, 1\}^{N \times K}$
\begin{align}\label{eq:prob_sort_hard}
	\mathbb{P}(P = P^*) = \prod\nolimits_{i = 1}^{n} P_{i, S(i;P^*)},
\end{align}
where $S(i;P^*)$ is the cluster to which $P^*$ assigns $v_i$ (i.e., $P^*_{ix} = 1$ if and only if $x = S(i;P^*)$).

We say that an objective function $f: \mathcal{P} \rightarrow \mathbb{R}$ is \textit{expectation-conforming}\footnote{Recently, similar properties have been discussed for set-functions~\cite{karalias2020erdos,karalias2021neural}.} if
\begin{align}\label{eq:goodprop}
	f(P) = \sum\nolimits_{P^* \in \mathcal{P}^*} \mathbb{P}(P = P^*) f(P^*), \forall P \in \mathcal{P}.
\end{align}
The intuitive is that, if $f$ satisfies Eq.~\eqref{eq:goodprop}, then for each (soft) cluster assignment matrix $P$, the value of $f$ directly taken on $P$ is equal to the \textit{expectation} of the value of $f$ when we see $P$ as a random variable taking values in $\mathcal{P}^*$.

\begin{lemma}\label{lem:exp_conf_no_local_min}
    \red{If $f: \mathcal{P} \rightarrow \mathbb{R}$ is expectation-conforming, then $f$ is linear w.r.t $(\mathbb{P}(P = P^*))_{P^* \in \mathcal{P}^*}$ and thus each local minimum is a global one.
    Moreover, let $\mathcal{P}^*_{min}$ denote the set of global minima of $f$ on $\mathcal{P}^*$.
    % For each global minima $P_{min}$ of $f$ on $\mathcal{P}$,
    % $\sum_{P^* \in \mathcal{P}^*_{min} \mathbb{P}(P_{min} = P^*)} = 1$.
    Also, $f$ satisfies the entry-wise concavity which guarantees that obtaining a deterministic $P^*$ from a soft $P$ does not decrease the performance~\cite{wang2022unsupervised}.} 
\end{lemma}

Recall the two different forms of objective functions:
\begin{itemize}
    \item \textbf{Modularity}. $f_Q(P) = -\frac{1}{2|E|}\sum_{i,j} (A_{ij} - \frac{d_i d_j}{2|E|})(P_i \cdot P_j)$;
    \item \textbf{Normalized cut}. $f_C(P) = -\frac{\operatorname{Tr}(P^{T}\tilde{A}P)}{\operatorname{Tr}(P^{T}\tilde{D}P)}$.
\end{itemize}
\begin{lemma}\label{lem:mod_exp_conf}
    Given any $G$, $f_Q$ is expectation-conforming.
\end{lemma}
% \vspace{-2mm}
\begin{proof}
    % We write $f_Q$ in a more general form, $f_Q(P) = \alpha \sum_{i, j} \beta_{ij} P_i \cdot P_j$, where $\alpha$ and $\beta_{ij}$'s are constants possibly depending on $G$.
    Since $\frac{1}{2|E|}$ and $(A_{ij} - \frac{d_i d_j}{2|E|})$'s are constants when $G$ is fixed, by the linearity of expectation~\cite{alon2016probabilistic}, suffice it to show that
    $P_i \cdot P_j = \sum_{P^* \in \mathcal{P}^*} \mathbb{P}(P = P^*) P^*_i \cdot P^*_j$.
    Indeed, RHS $= \sum_{P^* \in \mathcal{P}^*: P^*_i = P^*_j} \mathbb{P}(P = P^*) = \mathbb{P}(P \in \{P^* \in \mathcal{P}^*: P^*_i = P^*_j\}) = \sum_{x = 1}^{K} P_{ix} P_{jx} =$ {LHS}.
%     Given a soft cluster assignment matrix $P$, the probability of two nodes $v_i$ and $v_j$ being assigned to the same cluster, denoted by $\delta_{ij}(P^{\boldsymbol{w}})$, is $P^{\boldsymbol{w}}_i \cdot P^{\boldsymbol{w}}_j$.
%     The key point is that $\delta_{ij}(P^{\boldsymbol{w}}) = \sum_{P^* \in \mathcal{P}} \mathbb{P}(P^{\boldsymbol{w}} = P^*) \delta_{ij}(P^*)$.
%     \blue{FC: Details.}
% 	Hence, $L(\boldsymbol{w}) = L(P^{\boldsymbol{w}}) = \sum_{i, j} L^{\boldsymbol{w}}_{ij} = -\frac{1}{2M} \sum_{i, j} (A_{ij} - \frac{d_i d_j}{2M})$.
\end{proof}
\begin{lemma}\label{lem:ncut_not_exp_conf}
    $f_C$ is not expectation-conforming in general.
\end{lemma}
\vspace{-2mm}
\begin{proof}
    We expand $f_C$ as $f_C(P) = -\frac{\sum_{i, j}(P_i \cdot P_j)\tilde{A}_{ij}}{\sum_{i} (P_i \cdot P_i)\tilde{D}_ii}$.
    Consider a simple case where $G$ consists of two nodes and one edge between them with $K = 2$.
    We have $f_C(P) = -\frac{2 P_1 \cdot P_2}{P_1 \cdot P_1 + P_2 \cdot P_2} \neq
    \sum_{P^* \in \mathcal{P}^*} \mathbb{P}(P = P^*) f_C(P^*) = P_{11} P_{21} f_C((\begin{smallmatrix}1 & 0\\ 1 & 0\end{smallmatrix})) + P_{12} P_{22} f_C((\begin{smallmatrix}0 & 1\\ 0 & 1\end{smallmatrix})) = -P_{11} P_{21} - P_{12} P_{22} = -P_1 \cdot P_2$.
    The counterexamples when $G$ has more nodes or edges can be constructed similarly.
\end{proof}
% Notably, the normalized cut objective used by \MinCutPool~\cite{bianchi2020spectral} does not satisfy the property.
% \blue{FC: add it into the lemma?}
